From Randomized Response to Randomized Index: Answering Subset Counting Queries with Local Differential Privacy

Local Differential Privacy (LDP) is the predominant privacy model for safeguarding individual data privacy. Existing perturbation mechanisms typically require perturbing the original values to ensure acceptable privacy, which inevitably results in value distortion and utility deterioration. In this work, we propose an alternative approach -- instead of perturbing values, we apply randomization to indexes of values while ensuring rigorous LDP guarantees. Inspired by the deniability of randomized indexes, we present CRIAD for answering subset counting queries on set-value data. By integrating a multi-dummy, multi-sample, and multi-group strategy, CRIAD serves as a fully scalable solution that offers flexibility across various privacy requirements and domain sizes, and achieves more accurate query results than any existing methods. Through comprehensive theoretical analysis and extensive experimental evaluations, we validate the effectiveness of CRIAD and demonstrate its superiority over traditional value-perturbation mechanisms.

==> meta-review.tex <==
\newpage % The Meta-Review should at least start on a new column

% Use \appendices and not \appendix due to IEEEtran.cls quirks
\appendices % if not used earlier

\section{Meta-Review}

The following meta-review was prepared by the program committee for the 2025
IEEE Symposium on Security and Privacy (S\&P) as part of the review process as
detailed in the call for papers.

\subsection{Summary}
This paper introduces CRIAD (Counting via Randomized Index with Augmented Dummies), a novel Local Differential Privacy (LDP) mechanism for answering subset counting queries on set-value data. CRIAD uses a multi-dummy, multi-sample, and multi-group approach to balance accuracy and privacy.

\subsection{Scientific Contributions}
\begin{itemize}
	\item Independent Confirmation of Important Results with Limited Prior Research
	\item Provides a Valuable Step Forward in an Established Field
	\item Establishes a New Research Direction
\end{itemize}

\subsection{Reasons for Acceptance}
\begin{itemize}
	\item CRIAD outperforms SOTA approaches like kRR and RAPPOR by up to 30\% in accuracy.
	\item It guarantees $\epsilon$-LDP while producing unbiased subset count estimations.
	\item Conclusive experiments
\end{itemize}

\subsection{Noteworthy Concerns} % Exclude if your meta-review does not have noteworthy concerns
\begin{itemize} % Enumerate environment is not necessary if there is only one
	\item Reduced performance at low privacy budgets	
\end{itemize}

%\section{Response to the Meta-Review} % Optional
%
%%Less than 500 words response to the meta-review. The response to the meta-review is optional. Provide a response if you disagree with the meta-review. Shepherds will only deny responses to meta-reviews if they are too long or are abusive / inappropriate.
%
%Dear Reviewers,
%
%We are very grateful for your constructive comments, which have inspired us to improve our work. We have now revised our paper to address the following three noteworthy concerns, and we are seeking to have them removed. The modifications are highlighted in blue in the revised manuscript as attached. 
%
%**Excessively complex parameter tuning**: 
%We would like to clarify that the parameter selection of CRIAD (i.e., including $m$, $s$, and $g$) is automatically decided by Theorem 4.7. Solving Eq. 15 of Theorem 4.7 can be simplified by following two steps: (1) randomly sampling a portion of users to estimate $\pi_t$; and (2) enumerating all combinations of $m, s, g\in \mathbb{Z}^{+}$ and finding the one with the lowest variance. 
%
%Notably, in Step (1) each user only needs to report an integer, resulting in the whole process very efficient. In Step (2), $s$ and $g$ are typically small integers even for a large domain, as an increasing $s$ consumes privacy budget very quickly and a larger $g$ leads to significant sampling variance. As such, the number of combinations will not be too large. To simplify this process, we can conduct a greedy search to enumerate all combinations, calculate their resulted variance by Eq. 15, and select the optimal one with the lowest variance. 
%
%Now we have revised the last paragraph of Section 4.4 by removing the process of integer optimization and adding the above clarification to simplify the parameter setting of CRIAD, as highlighted in blue in the revised manuscript.  
%
%**Unclear scalability to very large datasets and communication overhead**:
%As for the scalability to large datasets, we would like to argue CRIAD demonstrates excellent scalability with very large datasets, as noted by Reviewer \#676A with comments --- ``They also demonstrate the scalability of CRIAD, showing its ability to handle larger datasets without compromising on performance''. Our study utilized datasets encompassing a large user population of up to 990,002 and a large item domain of up to 41,270. Regarding category size, although it does not exceed 1,600, Figure 3 illustrates that the performance gap between CRIAD and existing methods becomes more pronounced as the category size increases. This suggests that CRIAD scales effectively with larger category sizes. We have now revised the second paragraph of Section 5.3 to clarify this point. 
%
%As for communication overhead, each user is responsible for only one of $g$ groups and randomly reports $s$ bits to the server. Typically, $s$ is quite small. For instance, in Table 6, when $d=400$ and $\epsilon=1$, $s$ is set to $1$ in most cases. To reduce the cost of user coordination on server side, we have now revised Algorithm 3 and corresponding description (with modifications highlighted in blue) by allowing each user to randomly sample a group for reporting. Note that this will not cause any negative impact on the accuracy of CRIAD. Consequently, the server only needs to broadcast $(m,s,g)$ to all users. In a word, the communication overhead of CRIAD is kept in a healthy level, i.e., $s$ bits from each user to the server and 3 integers (of $m$, $s$, and $g$) from the server to all users.
%
%**Reduced performance at low privacy budgets**: 
%We would like to clarify that the reduced performance at low privacy budgets is due to significant perturbation required to ensure privacy, a challenge common to all existing LDP methods. Nevertheless, CRIAD demonstrates the most substantial improvement over existing methods at low privacy budgets. As illustrated in Figure 2, with a privacy budget of $\epsilon=0.1$, CRIAD outperforms the second-best method (i.e., RR) by a factor of at least 5 across different settings. 
%This is also noted by Reviewer \#676D with comments --- ``this approach gives very large improvement over the extant literature even at very small epsilons''.
%
%Now we have revised the first paragraph of Section 5.2 to further clarify this point, as highlighted in blue.





